Photospheric emission from GRB 211211A altered by a strong radiation-mediated shock

Gamma-ray burst (GRB) spectra are typically non-thermal, with many including two spectral breaks suggestive of optically-thin emission. However, the emitted spectrum from a GRB photosphere, which includes prior dissipation of energy by radiation-mediated shocks (RMSs), can also produce such spectral features. Here, we analyze the bright GRB 211211A using the Kompaneets RMS Approximation (KRA). We find that the KRA can fit the time-resolved spectra well, significantly better than the traditionally used Band function in all studied time bins. The analysis of GRB 211211A reveals a jet with a typical Lorentz factor ($\Gamma \sim 300$), and a strong RMS (upstream dimensionless specific momentum, $\gamma_u \beta_u \sim 3$) occurring at a moderate optical depth ($\tau \sim 35$) in a relatively cold upstream ($\theta_u = k_{\rm B} T_u / m_e c^2 \sim 10^{-4}$). We conclude that broad GRB spectra that exhibit two breaks can also be well explained by photospheric emission. This implies that, {in such cases}, the spectral shape in the MeV-band alone is not enough to determine the emission mechanism during the prompt phase in GRBs.

==> Preamble/packages.tex <==

\usepackage{graphicx}

\usepackage{amsmath}
\usepackage{comment}    % Allows for commenting out blocks of text
\usepackage{amssymb}
\usepackage{array}


\makeatletter
\renewcommand\hyper@natlinkbreak[2]{#1}
\makeatother

\makeatletter
\patchcmd{\ltx@foottext}{%
  .5\textwidth\advance\hsize-18pt}{%
  \linewidth\advance\hsize-1.8em%
}{}{}
\makeatother

\usepackage[T1]{fontenc}

